Distributed Stochastic Optimization of a Neural Representation Network for Time-Space Tomography Reconstruction

4D time-space reconstruction of dynamic events or deforming objects using X-ray computed tomography (CT) is an important inverse problem in non-destructive evaluation. Conventional back-projection based reconstruction methods assume that the object remains static for the duration of several tens or hundreds of X-ray projection measurement images (reconstruction of consecutive limited-angle CT scans). However, this is an unrealistic assumption for many in-situ experiments that causes spurious artifacts and inaccurate morphological reconstructions of the object. To solve this problem, we propose to perform a 4D time-space reconstruction using a distributed implicit neural representation (DINR) network that is trained using a novel distributed stochastic training algorithm. Our DINR network learns to reconstruct the object at its output by iterative optimization of its network parameters such that the measured projection images best match the output of the CT forward measurement model. We use a forward measurement model that is a function of the DINR outputs at a sparsely sampled set of continuous valued 4D object coordinates. Unlike previous neural representation architectures that forward and back propagate through dense voxel grids that sample the object's entire time-space coordinates, we only propagate through the DINR at a small subset of object coordinates in each iteration resulting in an order-of-magnitude reduction in memory and compute for training. DINR leverages distributed computation across several compute nodes and GPUs to produce high-fidelity 4D time-space reconstructions. We use both simulated parallel-beam and experimental cone-beam X-ray CT datasets to demonstrate the superior performance of our approach.

==> figs/deben202310/sec_apdx_ablation.tex <==
\section{Detailed Architecture and Training}
A detailed schematic of the network architecture 
for DINR is shown in Fig. \ref{fig:nnarch_train} (a).
The overall training loop for DINR
is shown in Fig.  \ref{fig:nnarch_train} (b).

\begin{figure}[h]
\centering
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/Supp_NN_Arch.png}
\caption{Detailed network architecture for DINR.}
\end{subfigure} \\
\hfill
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/Supp_Train_Loop.png}
\caption{Training loop for DINR.}
\end{subfigure}
\caption{Network architecture and training loop for DINR.}
\label{fig:nnarch_train}
\end{figure}

\section{Ablation Studies}\label{secA1}

In this section, we present ablation studies by performing several experiments to provide a more comprehensive understanding of our DINR reconstruction method. 


\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_ablation_arange.pdf}
\caption{ISO for first/last time frames.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.38\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_ablation_arange_psnr.pdf}
\caption{PSNR vs. angular range.}
\end{subfigure}
\caption{Effect of the rotation angular ranges on the reconstruction quality using our proposed DINR. (a) Isosurface 3D rendering of the first and last frame reconstructions for the rotation ranges shown in the row labels. (b) PSNRs of the reconstruction as a function of the different angular ranges.}
\label{fig:ablation_arange}
\end{figure}


\subsubsection*{Effect of Angular Ranges}

When the rotation angular range is limited, 
the projection data is incompletely sampled.
This results in a poor reconstruction that is
plagued by significant artifacts. 
In the case of MPM-simulated datasets 
where rapid deformation occurs, 
it is considered severely limited-angle 4DCT 
even though the total rotation range is 360\degree. 
In this ablation study, we performed our DINR reconstruction 
for different angular ranges of the projection data 
to observe the reconstruction performance. 
As shown in Figure~\ref{fig:ablation_arange}, 
the reconstruction quality remains satisfactory 
even up to a low angular range of 225\degree. 



\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_ablation_noise.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.38\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_ablation_noise_psnr.pdf}
\end{subfigure}
\caption{Effect of noise in projection data on the quality of reconstruction using our proposed DINR. (a) Isosurfaces of the reconstructed first and last frames for different noise levels specified in the row labels. (b) PSNRs of the reconstruction as a function of the noise percentages.}
\label{fig:ablation_noise} 
\end{figure}



\subsubsection*{Effect of Noise in Projection Data}
For our reconstruction results, we simulated CT 
projection data of the MPM-simulated datasets 
with a default noise level of 0.1\%. 
We simulate Poisson noise in the X-ray transmission space
(negative logarithm of projections).
In this ablation study, we simulated 
different noise levels for the projection data 
to investigate the robustness of our DINR method. 
Noise was added to the projection data 
at 6 different noise levels: 0, 1, 2, 4, 8, 16\%, 
as shown in Fig~\ref{fig:ablation_noise}. 
We observe that the reconstruction quality 
remains satisfactory up to a noise level of 2\%. 


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/figure_MPM_ablation_sigma.pdf}
\caption{Effect of different combinations of the GRFF parameters, $\sigma_s$ and $\sigma_t$, on the quality of reconstruction using DINR.}
\label{fig:ablation_sigma}
\end{figure}


\subsubsection*{Effect of GRFF Parameters}

$\sigma_t$ and $\sigma_s$ are application-specific 
bandwidth parameters used by the 
Gaussian Random Fourier Features (GRFF) of DINR
to control the temporal and spatial smoothness respectively
for the 4D reconstruction.
These parameters function as regularization parameters. 
A careful selection of $\sigma_s$ and $\sigma_t$ parameters 
may be required to obtain an optimal reconstruction quality.
While an optimal setting for $\sigma_s$ and $\sigma_t$ 
varies depending on the scene, we observed that  
$\sigma_t$ ranging from $0.01$ to $0.1$ 
and $\sigma_s$ ranging from $0.1$ to $0.5$ yield 
reasonably good reconstruction quality for the MPM-simulated datasets. 
Figure~\ref{fig:ablation_sigma} shows 4D reconstructions
using DINR for different combinations of $\sigma_t$ and $\sigma_s$.



==> figs/deben202310/sec_apdx_result.tex <==

\section{More Reconstruction Results}\label{secB1}

In this section, we show more reconstruction results of the MPM-simulated datasets that we did not include in the main paper. 


\begin{figure}
\centering

\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S03_001.pdf}
    \caption{S03\_001}
\end{subfigure}
\\
\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S03_008.pdf}
    \caption{S03\_008}
\end{subfigure}

\caption{4D reconstruction of the MPM-simulated dataset: S03\_001 (a) and S03\_008 (b). From \textit{left} to \textit{right}, $T_{0}, T_{20}, T_{40}, T_{60}, T_{80}, T_{90}$, respectively. Values indicates the averaged PSNR over frames.}
\end{figure}


\begin{figure}
\centering

\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S04_009.pdf}
    \caption{S04\_009}
\end{subfigure}
\\
\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S04_018.pdf}
    \caption{S04\_018}
\end{subfigure}

\caption{4D reconstruction of the MPM-simulated dataset: S04\_009 (a) and S04\_018 (b). From \textit{left} to \textit{right}, $T_{0}, T_{20}, T_{40}, T_{60}, T_{80}, T_{90}$, respectively. Values indicates the averaged PSNR over frames.}
\end{figure}


\begin{figure}
\centering

\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S05_700.pdf}
    \caption{S05\_700}
\end{subfigure}
\\
\begin{subfigure}[b]{0.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/figure_MPM_512_128_results_S08_005.pdf}
    \caption{S08\_005}
\end{subfigure}

\caption{4D reconstruction of the MPM-simulated dataset: S05\_700 (a) and S08\_005 (b). From \textit{left} to \textit{right}, $T_{0}, T_{20}, T_{40}, T_{60}, T_{80}, T_{90}$, respectively. Values indicates the averaged PSNR over frames.}
\end{figure}


==> figs/deben202310/sec_conclusion.tex <==

\section{Conclusion}

We formulated a novel approach called 
distributed implicit neural representation (DINR) for 
4D time-space reconstruction of objects 
imaged using X-ray computed tomography.
DINR is primarily composed of a fully-connected neural network
that is trained to reconstruct the X-ray attenuation properties 
of the object at its output as a function of the time-space coordinates. 
For training the DINR network, we presented a novel stochastic 
distributed optimization algorithm with near-linear scaling capability 
as a function of the number of GPUs.
DINR is capable of producing large sized terabyte sized 
4D reconstructions at high spatial and temporal resolutions.
Using 4DCT experimental data, we demonstrated that only DINR is
able to clearly resolve crack propagation in a SiC sample
and reconstruct the fine interleaving strands of a log-pile sample. 
We used the PSNR and SSIM performance metrics applied on
both simulated and experimental
data to quantitatively demonstrate the advantage of DINR when 
compared to state-of-the-art 4DCT reconstruction methods.



==> figs/deben202310/sec_discuss.tex <==

\section{Discussion}\label{sec12}

DINR is a function approximator that expresses the
linear attenuation coefficient (LAC)
as a continuous function of the 
object's 4D time and space coordinates.
Since the output of DINR is a continuous function in time-space,
it is inherently resistant to reconstruction of discontinuous 
artifacts such as streaks and noise unlike discrete voxel representations.
The state-of-the-art approaches to experimental
4DCT reconstruction assume a static object for the duration 
of projections used to reconstruct one volumetric time frame.
In this case, limited angle artifacts manifest 
as spurious streaks when the 
ratio of the angular rotation for the projections 
to the number of time frames is low.
These spurious artifacts rotate 
with the changing angular direction of X-rays across view angles
and are the primary reason for limiting the
temporal resolution of conventional 4DCT.
In contrast, DINR inherently assumes a dynamic object that
changes continuously over time and between subsequent projection images.
This allows DINR to achieve an order-of-magnitude higher
temporal resolution approaching the time duration 
for acquiring a single projection image.
This capability of DINR is revolutionary since it allows 
4D imaging of very fast dynamic systems or objects.

During each iteration of training, we only sample
a small subset of projection pixels to compute 
the updated values of the network parameters.
Then, we forward and back propagate through 
the DINR network at randomly sampled coordinates that lie 
along the ray paths connecting the projection pixels to the source.
This approach to training is highly memory and compute efficient
since it does not require instantiating and computing the values at
voxels that span the complete space-time object coordinates.
We discretize the space-time coordinates only during inference
and compute the reconstructed values at the discrete voxels
on a 4D time-space grid. 
While it may appear that neural network inference is memory 
intensive, this memory is only allocated on hard disk drives 
that are typically very large in size (up to terabytes). 
In contrast, training utilizes GPU memory that is typically
very limited (up to few tens of gigabytes). 

While we can produce a reconstruction 
from the DINR at any arbitrary time instant,
we do not expect a higher time resolution than
the time gap between two adjacent projection images (or view angles).
Similarly, we do not expect a higher spatial resolution
than the size of each detector pixel 
that is back projected onto the object plane.
Thus, we only sample and voxelize at the time instants of each projection view
and at a spatial resolution equal to the detector pixel size
divided by the geometric magnification.
The geometric magnification is one for parallel-beam 
and is the ratio of the source-to-detector distance and
the source-to-object distance for cone-beam geometry. 

DINR is a compressed representation of the temporal and
spatial distribution of the LAC for the scanned object.
Information on this 4D reconstruction is encoded 
in the parameters of the DINR network. 
The number of network parameters is an order of magnitude less
than the number of discrete voxels across time-space.
For the log-pile and SiC samples, 
the numbers of voxels are approximately 
$3\times 10^{11}$ and $7\times 10^{10}$ respectively.
However, the number of network parameters that reconstruct
the values at these voxels is approximately $8\times 10^4$.

==> figs/deben202310/sec_forward.tex <==

\section{Forward Model}
In a X-ray CT scanner, 
the propagation direction of X-rays 
is defined by the so-called geometry of the scanner, 
which is a function of the position and orientations 
of the X-ray source and detection system.
We consider three X-ray scanner geometries 
including cone-beam, fan-beam, and 
parallel-beam geometry.
For the detector, 
we use a scintillator-based detection 
system that is modeled as a 2D panel consisting
of a rectilinear grid of sensor pixels 
with finite area. 

\begin{figure}[!thb]
\begin{center}
\includegraphics[width=4in]{figs/geometry.png}
\end{center}
\caption{\label{fig:geomdiag}
}
\end{figure}

\begin{figure}[!thb]
\begin{center}
\includegraphics[width=4.5in]{figs/rotation.png}
\end{center}
\caption{\label{fig:rotdiag}
}
\end{figure}

The measured CT data is a function of the time-space 
distribution of the linear attenuation coefficient 
(LAC), denoted by $\mu([t,z,y,x]^T)$, of the object.
Here, $t$, $z$, $y$, and $x$ are the time, 
$z$-axis, $y$-axis, and $x$-axis world 
coordinates respectively.
The LAC is a measure of the amount of X-ray
attenuation caused by various material
interaction properties such as photoelectric
absorption and scatter. 
For any detector pixel indexed by $(i,j)$,
the measurement is an average of the 
X-ray intensities along a continuum 
of rays that originate from the 
point-source, propagate through the object, and
end at a location inside the 
pixel's surface area.
Here, the row and column indices of a 
detector pixel are denoted by 
$i$ and $j$ respectively. 
Let the set of all coordinates within the 
surface area of the detector pixel $(i,j)$
be given by,
\begin{multline}
    C_{i,j} = \left\lbrace (x_d, z_d) \,\vert\, 
    -C_x + i\Delta_x \leq x_d < -C_x + (i+1)\Delta_x,\right.\\
    \left. -C_z + j\Delta_z \leq z_d < -C_z + (j+1)\Delta_z
    \right\rbrace,
\end{multline}
where $x_d$ and $z_d$ are the $x$-axis 
and $z$-axis coordinates on the detector plane,
and $\Delta_x$ and $\Delta_z$ are the widths 
of the detector pixel along the $x$-axis 
and $z$-axes respectively.
Here, $C_x$ and $C_z$ are the distances
of the optical axis from the left-vertical and 
bottom-horizontal edges of the detector panel. 

The measurement made by detector pixel $(i,j)$
is a direct measure of the linear projections 
of the LAC $\mu([x,y,z,t]^T)$ along rays that
connect the X-ray source to points on the
surface of the pixel $(i,j)$.
The $y$-axis is defined along the optical axis, 
which is the ray originating at the X-ray source
and intersecting perpendicularly at the detector.
Without loss of generality, 
the $x$-axis coordinate for the optical axis
is $x=0$ and $y=0$ is the center of 
rotation for the object along the $y$-axis.
The center of rotation for the object
along the $x$-axis is denoted by $x_{s0}$.
The object is rotated along the $z$-axis
and $z=0$ marks the center of the object
along the $z$-axis. 
To rotate the source and detector coordinates
in the $x-y$ axial plane by an 
anti-clockwise angle of $\theta_k$, we use the 
following equations,
\begin{align}
    x_{s,k} & = x_s \cos\left(\theta_k\right) - y_s \sin\left(\theta_k\right) + \left(x_{s0} -
      x_{s0}\cos\left(\theta_k\right)\right),  \label{eq:rotxsk}\\
    y_{s,k} & = x_s \sin\left(\theta_k\right) 
      + y_s \cos\left(\theta_k\right)
      - x_{s0}\sin\left(\theta_k\right), \label{eq:rotysk}\\
    x_{d,k} & = x_d \cos\left(\theta_k\right) - y_d \sin\left(\theta_k\right) + \left(x_{s0} -
      x_{s0}\cos\left(\theta_k\right)\right), \text{ and } \label{eq:rotxdk} \\
    y_{d,k} & = x_d \sin\left(\theta_k\right) 
      + y_d \cos\left(\theta_k\right)
      - x_{s0}\sin\left(\theta_k\right).\label{eq:rotydk}
\end{align}
Anti-clockwise rotation of source and detectors 
by an angle of $\theta_k$ is equivalent to clockwise
rotation of object coordinates by $\theta_k$.

The linear projection of the LAC, $\mu(\cdot)$, 
along a ray that connects
the X-ray source at $[x_s, y_s, z_s]^T$ and 
a detector coordinate at $[x_d, y_d, z_d]^T$ 
at time $t=t_k$ is,
\begin{multline}
    p\left(\begin{bmatrix}
    x_d \\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s \\ y_s \\ z_s
    \end{bmatrix}, 
    \begin{bmatrix}
    t_k \\
    \theta_k
    \end{bmatrix}
    \right) =
    \int_{\delta=\delta_{min}}^{\delta_{max}} 
    s\left(\begin{bmatrix}
    x_d\\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s\\ y_s \\ z_d
    \end{bmatrix}\right)\\
    \mu\left(\begin{bmatrix}
    x_{s,k} \\ y_{s,k} \\ z_s \\ t_k
    \end{bmatrix}
    + \delta
    \begin{bmatrix}
    x_{d,k}-x_{s,k} \\ 
    y_{d,k}-y_{s,k} \\ 
    z_d-z_s \\
    0
    \end{bmatrix}\right)
    d\delta,
    \label{eq:parlineint}
\end{multline}
where $\delta$ is used to parameterize 
the line connecting 
$[x_s,y_s,z_s]^T$ and $[x_d,y_d,z_d]^T$.
The limits of the integral, 
$\delta_{min}$ and $\delta_{max}$,
mark the outer boundary of the object.
Thus, the LAC is zero for 
$\delta<\delta_{min}$ or $\delta>\delta_{max}$.
We assume that the object is stationary for the 
duration of the detector's exposure time. 
The arc-length is given by,
\begin{equation}
\label{eq:arclength}
s\left(\begin{bmatrix}
    x_d\\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s\\ y_s \\ z_d
    \end{bmatrix}\right) 
    = \left\vert\left\vert
    \begin{bmatrix}
    x_d\\ y_d \\ z_d
    \end{bmatrix}
    - \begin{bmatrix}
    x_s\\ y_s \\ z_s
    \end{bmatrix}
    \right\vert\right\vert^2_2.
\end{equation}
The source-to-object distance is 
$\vert y_s \vert$
and object-to-detector distance is 
$\vert y_d \vert$.

For each $(i,j,k)$, we compute several 
line integrals using equation \eqref{eq:parlineint} 
along the lines that connect the X-ray source 
to several locations on the finite sized 
detector pixel and average the line integrals
within each pixel. 
The measurement at detector pixel $(i,j)$ is,
\begin{equation}
\label{eq:beerstransavg}
    I_{i,j,k} = I^{(0)}_{i,j,k}\int_{(x_d,z_d)\in C_{i,j}}
    \exp\left\lbrace
    -p\left(\begin{bmatrix}
    x_d \\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s \\ y_s \\ z_s
    \end{bmatrix}, 
    \begin{bmatrix}
    t_k \\
    \theta_k
    \end{bmatrix}\right)
    \right\rbrace
    dx_d dz_d,\\
\end{equation}
where $I^{(0)}_{i,j,k}$ is the X-ray intensity 
in the absence of the object.
We approximate equation \eqref{eq:beerstransavg}
by moving the integration to within the exponential,
which is useful to formulate a linear forward model
that reduce the computational cost. 
Thus, our model for the measurement is,
\begin{equation}
\label{eq:beersattenavg}
    I_{k,i,j} = I^{(0)}_{k,i,j}\exp
    \left(-\int_{(x_d,z_d)\in C_{i,j}}
    p\left(\begin{bmatrix}
    x_d \\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s \\ y_s \\ z_s
    \end{bmatrix}, 
    \begin{bmatrix}
    t_k \\
    \theta_k
    \end{bmatrix}\right)
    dx_d dz_d\right).\\
\end{equation}

Our goal is to reconstruct $\mu([x,y,z,t]^T)$ from 
measurements $I_{i,j,k}$ using 
equation \eqref{eq:beersattenavg}.
Since equation \eqref{eq:beersattenavg} is non-linear, 
we use logarithms to obtain a relation that is 
linear in $\mu([x,y,z,t]^T)$.
Let $f_{i,j,k}\left(\mu(\cdot)\right)$ be the negative 
logarithm of the ratio between $I_{i,j,k}$ and $I_0(i,j,k)$.
Then, using the logarithmic transformation for 
equation \eqref{eq:beersattenavg}, we get,
\begin{multline}
\label{eq:logbeerslaw}
f_{i,j,k}\left(\mu\left(
\begin{bmatrix}
x\\ y\\ z\\ t
\end{bmatrix}
\right)\right) 
    =-\log\left\lbrace\frac{I_{i,j,k}}{I^{(0)}_{i,j,k}}\right\rbrace = \\
    \int_{(x_d,z_d)\in C_{i,j}}
    p\left(\begin{bmatrix}
    x_d \\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s \\ y_s \\ z_s
    \end{bmatrix}, 
    \begin{bmatrix}
    t_k \\
    \theta_k
    \end{bmatrix}\right)
    dx_d dz_d.
\end{multline}
In practice, we cannot measure $I^{(0)}_{i,j,k}$ at every $t_k$.
Instead, we acquire X-ray images without the object
at a few distinct time intervals and approximate 
$I^{(0)}_{i,j,k}$ from these images. 
Thus, the forward measurement model is,
\begin{equation}
\label{eq:forwmod}
y_{i,j,k} = f_{i, j, k}\left( 
\mu\left(\left[x, y, z,
t\right]^T\right)\right)
+ n_{i,j,k},
\end{equation}
where $n_{i,j,k}$ Poisson-like noise that 
is modeled as a Gaussian random variable with a
standard deviation of 
$\sqrt{f_{i, j, k}\left(\mu(\cdot)\right)}$.

To compute $f_{i,j,k}(\cdot)$, 
we need to numerically evaluate the integrals
in equations \eqref{eq:beersattenavg} 
and \eqref{eq:parlineint}.
For numerical integral calculation, 
we choose between either a regular equi-spaced 
sampling or randomized sampling for
$\delta$, $x_d$, and $z_d$.
For equi-spaced sampling, we regularly 
sample the detector coordinates
$(x_d, z_d) \in C_{i,j}$ with equal spacing
between adjacent samples along both $x$-axis and $z$-axis.
For each sampled $(x_d, z_d)$, we again perform 
equi-spaced sampling of the $\delta$ coordinate 
that parameterizes the line connecting the 
source to the detector pixel $(i,j)$.
For randomized sampling, we sample all the coordinates
of $\delta$, $x_d$, and $z_d$ uniformly at random.
Let $\Psi_{i,j,k}$ be the set of all sampled $(x_d, z_d, \delta)$
coordinates for the measurement at $(i,j,k)$.
Then, a numerical estimate for $f_{i,j,k}(\cdot)$
is given by,
\begin{multline}
    \hat{f}_{i,j,k}\left(\mu\left(
    \begin{bmatrix}
    x\\ y\\ z\\ t
    \end{bmatrix} \right)\right) =
    \frac{\left(\delta_{max}-\delta_{min}\right)}{\left\vert\Psi_{i,j,k}\right\vert}
    \sum_{(x_d,z_d,\delta)\in \Psi_{i,j,k}}
     s\left(\begin{bmatrix}
    x_d\\ y_d \\ z_d
    \end{bmatrix},
    \begin{bmatrix}
    x_s\\ y_s \\ z_d
    \end{bmatrix}\right)\\
    \mu\left(\begin{bmatrix}
    x_{s,k} \\ y_{s,k} \\ z_s \\ t_k
    \end{bmatrix}
    + \delta
    \begin{bmatrix}
    x_{d,k}-x_{s,k} \\ 
    y_{d,k}-y_{s,k} \\ 
    z_d-z_s \\ 0
    \end{bmatrix}\right).
    \label{eq:estforwmod}
\end{multline}
To compute $\hat{f}_{i,j,k}(\mu(\cdot))$, 
the limits for sampling of $x_d$, $z_d$, and $\delta$ 
are $\left(-C_x+i\Delta_x, -C_x+(i+1)\Delta_x\right)$,
$\left(-C_z+j\Delta_z, -C_z+(j+1)\Delta_z\right)$, and
$\left(l_{min}, l_{max}\right)$.
In equation \eqref{eq:estforwmod}, the summation
is over all the sampled values of $(x_d, z_d, \delta)$
in the region that connects the X-ray source source
to the surface area of the pixel $(i,j)$ 
at rotation angle $\theta_k$.
The samples of coordinates within this region 
for our integration by summation approach
is contained in the set $\Psi_{i,j,k}$.
In the next section, we substitute the LAC term,
$\mu(\cdot)$ in equation \eqref{eq:estforwmod}
with the neural representation 
network $\mathcal{M}_{\gamma}(\cdot)$.
Both $\mu(\cdot)$ and $\mathcal{M}_{\gamma}(\cdot)$
are functions of the world coordinates $(x,y,z,t)$.

==> figs/deben202310/sec_intro.tex <==

%\section{Introduction}\label{sec:intro}

%(Placeholder text for this section) 4D Time-Space Computed Tomography (4DCT) is an emerging imaging modality for non-destructive characterization of dynamic 3-dimensional (3D) objects in scientific imaging. 4DCT has been used for 3D reconstruction of the temporal dynamics in scientific imaging experiments such as dendritic solidification \cite{}, battery failure degration \cite{}, etc. 
%In X-ray CT, an object is rotated along an axis and measurements are acquired at several view angles of the rotating object. The popular approaches to CT reconstruction rely on an assumption of static object for the duration of several projections over a wide angular range of rotation (say $180^0$). Thus, the time axis is split into several contiguous non-overlapping frames and one 3D volume is reconstructed using the projection data within each frame.
% In reality, however, the object changes continuously from view-to-view due to the temporal evolution of the dynamic object. Hence, the current approaches for 4DCT are applicable only if the temporal evolution is sufficiently slow to make an assumption of static object within the duration of a single frame. This is a major limitation of existing 4DCT approaches since it imposes a lower limit on the achievable temporal resolution that is equal to the frame duration.

\section{Introduction}
\IEEEPARstart{X}{-ray} computed tomography (CT) is a widely used imaging modality for 
non-destructive characterization in industrial and scientific imaging, 
clinical diagnosis in medical imaging, 
and border security at airports. 
It is useful to produce 3D object reconstructions from 
X-ray projection images at several view angles 
around the object. 
Tomographic 3D reconstruction from its projection 
images is a linear inverse problem with numerous solutions 
that include analytical back-projection methods ~\cite{kak1998},
iterative algorithms, and deep learning approaches ~\cite{wang2020}. 
Unlike conventional CT, 4D time-space CT (4DCT) is an 
emerging imaging modality that is useful 
for reconstruction of dynamic objects.
However, 4DCT poses an extremely challenging and ill-posed inverse problem 
since the X-ray projection images are snapshots of a 
continuously time varying 3D scene or object.
4DCT has been used for 
studying in-situ object deformation under mechanical and thermal loading,
dendritic solidification ~\cite{gibbs2015three, mohan2015timbir}, 
battery failure degradation ~\cite{Kok_2023,ziesche20204d}, 
and periodic motion of the breathing phases in clinical diagnosis 
~\cite{taubmann2017spatio, schwemmer2013opening, schwemmer2013residual, rohkohl2008c, keall2004acquiring, pan20044d}. 
Several 4DCT methods have also been proposed to reconstruct 
non-periodic deforming scenes using 
motion field parameters ~\cite{zang2019warp, zang2018space}. 

In conventional X-ray CT, the 3D reconstruction approaches
rely on an assumption of a static object during 
the entire projection data acquisition. 
In 4DCT, however, the object is expected to change 
continuously over time and between subsequent views.
Such a temporal change may be attributed to several factors
including object motion, system instabilities, 
and dynamic physical processes such as due to to 
thermal or mechanical loading. 
The state-of-the-art (SOTA) approaches for 4DCT 
~\cite{zang2019warp, zang2018space, mohan2015timbir}
group the projection images into several frames such 
that each frame consists of consecutive projection images 
over an angular range of at least $180^{\circ}$.
The projection images in each frame is then reconstructed
into one 3D volume using tomographic reconstruction algorithms.

To avoid limited angle artifacts in the
reconstructed 3D volumes \cite{mohan2015timbir}, 
it is necessary to have a minimum of $180^{\circ}$ 
angular range of rotation in each frame.
Note that this requirement is essential for both 
static and dynamic CT.
The projections are grouped such that 
the temporal evolution is sufficiently slow 
to make an assumption of static object for the duration 
of each frame. 
This is a major limitation since it limits the achievable temporal 
resolution to the time duration of each frame. 
The significant temporal dynamics in many 4DCT experiments 
may lead to a rapidly changing object 
within the duration of each frame. 
Thus, existing reconstruction approaches for 4DCT 
produce inaccurate reconstructions that are
deteriorated by spurious artifacts and blurry features 
when the object changes rapidly within a frame.

Implicit neural representation (INR) networks,
also called neural radiance fields (NeRF), have demonstrated
remarkable potential in solving several inverse imaging problems. 
%such as view synthesis, object reconstruction, 
%object pose estimation, and other physics simulations. 
They have been successfully applied in several applications
including view synthesis  ~\cite{Mildenhall20eccv_nerf, riegler2020free, dupont2020equivariant, zhang2021neural, wang2022r2l}, 
texture completion ~\cite{chibane2020implicit}, 
deformable scene estimation ~\cite{park2020deformable, pumarola2020d}, 
and 3D reconstruction ~\cite{yariv2021volume, wang2021neus, meng_2023_neat}. 
INR networks behave as function approximators by representing
an object's physical properties as a differentiable 
function of the 3D spatial or temporal coordinates.
They are primarily composed of fully connected layers 
(multi-layer perceptron) whose parameters are trained to learn
an optimal mapping from coordinates to object properties.
This optimal map is learned by minimizing a loss function whose purpose
is to minimize the discrepancy between the measured data
and a forward model, which is a differentiable 
mathematical model for the sensor or detector data as a function
of the object properties.

In recent years, several INR-based approaches have been 
successfully applied to various CT reconstruction problems. 
For dynamic 4DCT reconstruction, an INR approach 
coupled with parametric motion fields has been proposed 
to reconstruct rapidly deforming scenes \cite{Reed2021}. 
This approach is useful for reconstruction of deforming objects
or periodic motions by optimizing both an object template and motion field parameters
used for representing the temporal dynamics by appropriate warping of the template.
While this approach significantly outperformed other state-of-the-art approaches, 
its implementation is prohibitively expensive in terms of the computational
and memory resource requirements for the Graphics Processing Units (GPUs).
This resource limitation is primarily due to forward and back propagation
through discrete voxel\footnote{Voxel is short-form for volume element
and is the 3D equivalent of a 2D pixel.} 
grids that fully instantiate the object properties across space and time.
Hence, this approach is infeasible for real-world use-cases
where it may not be possible to even store a 
single 3D voxelized volume in a GPU's memory.
For 4DCT, we may require storage of several hundreds of voxelized 
volumes that represent the object's dynamics over time. 
We estimate that thousands to tens of thousands of GPU resources may be required 
for 4DCT reconstructions of realistic experimental data that may span
gigabytes to terabytes in size.

In this paper, we present a novel reconstruction approach 
called Distributed Implicit Neural Representation (DINR) 
that uses a new distributed training algorithm for 
optimizing a continuous space-time representation for the object. 
DINR can scale to extremely large data sizes 
since it only uses a small number of randomly sampled projection pixel 
values for optimization of the network parameters in any training iteration.
For each randomly chosen projection pixel, DINR only
requires forward and back propagation through the network
at only those 4D object coordinates
that contribute to the sampled projection values.
Thus, the memory and compute requirements per GPU
for DINR is drastically lower than previous INRs since they
instantiate large sized voxel grids during training.
DINR learns to reconstruct the object in 4D at high-resolutions 
using multiple GPUs that are distributed over several nodes.
The number of sampled projection pixels can be adjusted to fit 
the maximum combined memory capacity of the available GPUs. 
Our approach can be run either on single GPU machines, 
multi-GPU workstations, or multi-node GPU clusters 
in high-performance computing (HPC) architectures. 
Next, we describe our 4DCT experimental setup
and our novel approach to 4D time-space reconstruction.

\begin{figure*}[!thb]
\begin{center}
\includegraphics[width=5in]{figs/Main-Figure.png}
\end{center}
\caption{\label{fig:mainfig}
Schematic of our distributed implicit neural representation 
(DINR) approach to 4DCT reconstruction.
The projection estimate $\bar{p}_i$ is a function of the 
linear attenuation coefficient (LAC) at coordinates
$r_{i,j}$ inside the orange colored 
pyramidal volume shown in (a, b).
The output of the DINR network, 
$\mathcal{M}(r_{i,j}; \gamma)$, gives the LAC 
at coordinate $r_{i,j}$.
(c) shows the loss function that is local
to each process and computed over a small subset 
$\Omega_k$ of projection indices.
For the projection image at the $m^{th}$ view,
the time $t_i$ for each projection pixel 
is the same value of $T_m$ since the time instant
for all pixels in an image must be the same.
(d) is our distributed approach
to training of the DINR network.
}
\end{figure*}

\section{Our Approach}
A schematic of our experimental setup for X-ray CT 
is shown in Fig. \ref{fig:mainfig} (a).
Here, a rotating object is exposed to X-ray radiation 
and images of the X-ray intensity 
after propagation through the object are acquired 
by a detector at several view angles of the object.
The detector is a panel of sensor pixels 
that are arranged in the form of a matrix.
While our approach is broadly applicable to 
a wide range of X-ray imaging systems,
we focus our discussion specifically on cone-beam and 
parallel-beam X-ray system geometries. 
In cone-beam geometry, X-rays are modeled as
originating from an infinitesimally small X-ray point source.
Alternatively, X-rays are modeled as parallel rays
when propagating from the source to the detector
in parallel-beam geometry.
Cone-beam is a more challenging geometry for reconstruction
since X-rays propagate in 3D unlike parallel-beam
where X-ray propagation is limited to a 2D plane.

The detector measurements are a function of the
temporal and spatial distribution of a material property called
linear attenuation coefficient (LAC) for the object.
A 4D reconstruction refers to estimation
of the LAC distribution for the object 
across space and time coordinates. 
Thus, the LAC is a function of the
4D continuous coordinates $r=(t,z,y,x)$, 
where $t$ is the time, 
and $(z,y,x)$ are the 3D spatial coordinates.
Let $p_i$ denote the $i^{th}$ projection such 
that $0 \leq i < MN$, where $M$ is the total number 
of tomographic views and $N$ is the number of detector pixels.
The projection $p_i$ is proportional to the negative logarithm of the 
sensor measurement at view index $\lfloor\frac{i}{N}\rfloor$ 
and detector pixel index $i \mod\left(N\right)$.
If $\lambda_i$ and $\bar{\lambda}_i$ are the sensor measurements
with and without the object respectively,
then $p_i=-\log\left(\lambda_i/\bar{\lambda}_i\right)$.

For any projection $p_i$ shown in Fig. \ref{fig:mainfig} (b),
we estimate its value $\bar{p}_i$ as the weighted sum of 
the LAC, $\mu(r)$, at time $t_i$ and 
spatial coordinates contained within the orange-colored 
pyramidal volume that connects the X-ray source
to the detector pixel that measures $p_i$.
Here, $t_{i}$ is the measurement time instant for $p_i$.
Since the object is also assumed to lie inside a cylinder-shaped 
field of view (FOV), only the coordinates within this FOV
contribute to the estimate $\bar{p}_i$.
Henceforth, we will refer to the intersection
of the pyramidal volume and the FOV as the 
region-of-influence for $p_i$.
Let $r_{i,j}=(t_{i},z_{i,j},y_{i,j},x_{i,j})$ 
be a coordinate sample such that $(z_{i,j},y_{i,j},x_{i,j})$ is 
contained in the region-of-influence for $p_i$.
We use a ray-sampling method for generating the coordinate 
samples, $(z_{i,j},y_{i,j},x_{i,j})$, that is described 
in the methods section \ref{sec:linproj}.
We refer to the computation of $\bar{p}_i$ from 
the LAC values, $\mu(r_{i,j})$, at several coordinates
samples, $r_{i,j}\, \forall j$, as the forward model.

To train the DINR network, 
we need a forward model that is a 
function of the outputs from the DINR network. 
The output of DINR, denoted by 
$\mathcal{M}(r_{i,j}; \gamma)$, is the LAC at 
the coordinate $r_{i,j}$ of the object.
Here, $j$ is an index for the samples of object coordinates $r_{i,j}$
within the region-of-influence for projection $p_i$.
The forward model as a function of $\mathcal{M}(r_{i,j}; \gamma)$ is 
$\bar{p}_i = \sum_j w(r_{i,j}) \mathcal{M}(r_{i,j}; \gamma)$.
Here, $w(r_{i,j})$ is a weight parameter 
that is a function of the spatial coordinates $(z_{i,j},y_{i,j},x_{i,j})$
and the imaging geometry. 
The formula for computation of $w(r_{i,j})$ 
is presented in the methods section \ref{sec:linproj}. 
$w(r_{i,j})$ has two distinct purposes that is 
described by factorizing $w(r_{i,j})$ as,
\begin{equation}
\label{eq:weightfactors}
w(r_{i,j})=\mu_0\l(r_{i,j}).    
\end{equation}
The first term $\mu_0$ is used to scale the output 
$\mathcal{M}(r_{i,j}; \gamma)$ of DINR to have units of LAC.
The purpose of $\mu_0$ is also to improve the convergence
speed of the training optimization loop.
It is set to be approximately equal 
to the average value of the object's LAC.
The second term $l(r_{i,j})$ is another scaling factor 
for the output $\mathcal{M}(r_{i,j}; \gamma)$
that is equal to the
length of the ray inside the cylindrical FOV that
connects the X-ray source to the detector pixel for $p_i$.
The expression $\sum_j w(r_{i,j}) \mathcal{M}(r_{i,j}; \gamma)$
is the unit-less linear projection of the LAC along the $i^{th}$ ray path.  

We train a DINR to reconstruct the LAC as a 
function of the object coordinates by minimizing a loss function
that is a measure of the distance between the projection data
and its predictions using the forward model.
The network parameters, denoted by $\gamma$, are iteratively
optimized such that the projection estimate $\bar{p}_i$ is progressively
driven closer to the measured projection $p_i$ for every $i$.
We define a L2 loss function that is a 
measure of the squared distance between $p_i$
and its estimate $\bar{p}_i$ as,
\begin{equation}
    \label{eq:mainsqdist}
    d_i(\gamma) = \left(p_i-\bar{p}_i\right)^2 
    = \left(p_i-\sum_j w(r_{i,j})\mathcal{M}(r_{i,j}; \gamma)\right)^2.
\end{equation}
Then, we train our DINR by estimating the $\gamma$ that
solves the following optimization problem,
\begin{equation}
    \label{eq:mainoptfunc}
    \hat{\gamma} = \arg\min_{\gamma} \frac{1}{MN}\sum_{i=1}^{MN} d_i(\gamma).
\end{equation}

Due to the compute and memory intensive nature of the 
minimization problem in \eqref{eq:mainoptfunc}, 
we solve it using distributed and stochastic optimization
over several compute processes.
The processes run on several GPUs distributed over
several compute nodes such that they collaboratively 
train the DINR to reconstruct the object.
Fig. \ref{fig:mainfig} (d) is a schematic of our approach to 
distributed optimization for learning of the 
network parameters $\gamma$.
In each process $k$, we randomly choose a subset $\Omega_k$
of projection indices $i$ from the set of $NM$ projection pixels.
As an example, the red-colored pixels in Fig. \ref{fig:mainfig} (c)
show the randomly chosen projection pixels whose indices
are contained in the set $\Omega_k$.
Then, we compute the local loss function 
$L\left(\Omega_k; \gamma\right)$ at each process $k$ 
such that it only sums the squared distances in \eqref{eq:mainsqdist}
over the small subset of indices $i\in\Omega_k$. 
The local loss function for each process is given by,
\begin{equation}
\label{eq:localoptfunc}
L\left(\Omega_k; \gamma\right)=
\frac{1}{\left\vert\Omega_k\right\vert}\sum_{i\in \Omega_k} d_i(\gamma),
\end{equation}
where $\vert\Omega_k\vert$ is the cardinality 
(number of elements) of the set $\Omega_k$.
Note that $\vert\Omega_k\vert$ is the batch size 
for process $k$ and is the same for all processes. 
Thus, if $K$ is the total number of processes, then 
the total batch size per iteration is,
\begin{equation}
\label{eq:totbatch}
\Omega_{*} = K\vert\Omega_k\vert.
\end{equation}
The batch size per GPU $\vert\Omega_k\vert$ is adjusted
based on the amount of memory in each GPU.

We use back-propagation to compute the local gradient, 
$\nabla_{\gamma}L\left(\Omega_k; \gamma\right)$, 
of $L\left(\Omega_k; \gamma\right)$ with respect to $\gamma$ in each compute process $k$ (Fig. \ref{fig:mainfig} (d)).
This local gradient function
$\nabla_{\gamma}L\left(\Omega_k; \gamma\right)$
includes only the back-propagation of the loss terms 
$d_i(\gamma)\,\forall i\in\Omega_k$. 
Then, the gradients from all the processes are averaged and 
the averaged gradient is broadcast back to each individual process $k$.
This averaged gradient is denoted as 
$\nabla_{\gamma}L\left(\Omega_*; \gamma\right)$,
where the set $\Omega_*$ includes the projection indices 
from all the subsets $\Omega_k \forall k$. 
Finally, the optimizer updates the parameters $\gamma$ 
within each process.
We use the Adam optimizer \cite{adam_opt_2015} for estimation of $\gamma$.
Our approach to distributed optimization is highly scalable
where distinct processes are run simultaneously 
on several hundreds of distinct GPUs.
Each process maintains a local copy of the DINR network 
$\mathcal{M}\left(r; \gamma\right)$ 
and uses its own instance of the optimizer for updating $\gamma$.
Since the optimizer in each process uses the same averaged gradient 
across all the processes, 
the parameter $\gamma$ after the update will also remain the same. 
One training epoch is the number of iterations
that is required to iterate over $MN$ number of projection pixels.
Thus, the number of iterations in each epoch 
is $\lceil\frac{MN}{\vert \Omega_{*}\vert}\rceil$
where $\Omega_{*}$ is the batch size from \eqref{eq:totbatch}.



==> figs/deben202310/sec_method.tex <==

\section{Methods}
\subsection{Linear Projection}
\label{sec:linproj}

\begin{figure}[!thb]
\begin{center}
\includegraphics[width=5in]{figs/Mtd-RaySum.png}
\end{center}
\caption{\label{fig:mtdraysum}
$\bar{p}_i$ is the weighted sum of $\mathcal{M}\left(r_{i,j}; \gamma\right)$
at equi-spaced coordinate samples on multiple ray traces 
from the X-ray source to the detector pixel 
that measures the projection $p_i$. 
The contribution of $\mathcal{M}\left(r_{i,j}; \gamma\right)$
to $\bar{p}_i$ is scaled by the length of the portion 
of the ray inside the region-of-influence that contains $r_{i,j}$. 
We show ray traces for cone-beam, 
parallel-beam, fan-beam,
and modular-beam geometries in (a), (b), (c), and (d) respectively.
}
\end{figure}

In this section, we present our approach to compute
$\bar{p}_i$ that is an estimate for the $i^{th}$ projection measurement
used in equation \eqref{eq:mainsqdist}.
To compute $\bar{p}_i$, we trace several rays 
from the X-ray source to the pixel that measures $p_i$
as shown in Fig. \ref{fig:mtdraysum}.
The end points of all the rays are equally spaced 
on a 2D grid over the surface of the $i^{th}$ pixel.
The 2D grid is obtained by equally sub-dividing each pixel 
into $D\times D$ number of sub-pixels and tracing rays to 
the centers of the sub-pixels. 
For a diverging cone-beam (Fig. \ref{fig:mtdraysum} (a)), the rays
originate from a single point source.
For parallel-beam (Fig. \ref{fig:mtdraysum} (b)), the rays
are mutually parallel.
We also show ray tracings for fan-beam
and modular-beam geometries in Fig. \ref{fig:mtdraysum} (c)
and Fig. \ref{fig:mtdraysum} (d) respectively.
However, we do not investigate reconstructions from 
fan-beam and modular-beam geometries in this paper.
Modular-beam is a generic specification
for defining the direction of X-ray propagation
that applies to any system geometry. 
To define the geometry, it uses known locations for the X-ray sources
and detector panels that can be placed at arbitrary coordinates in 3D space.

Along each ray in Fig. \ref{fig:mtdraysum}, 
we produce equi-spaced samples of coordinates
that are within the cylindrical region-of-influence for the object.
The spacing between adjacent coordinate samples
along each ray is $\Delta/D$, 
where $D$ is the up-sampling factor that is chosen as $D=2$.
We denote each coordinate sample as $r_{i,j}$.
Thus, the estimate $\bar{p}_i$ is given by,
\begin{equation}
    \bar{p}_i = \sum_j w(r_{i,j})\mathcal{M}(r_{i,j}; \gamma).
\end{equation}
Here, the weight term is given by 
$w(r_{i,j})=\mu_0 l(r_{i,j})$, where $l(r_{i,j})$ 
is the length of the ray inside the region-of-influence 
that contains the coordinate $r_{i,j}$.
We also use a scaling term 
$\mu_0$ that is approximately the average LAC value for the object. 
The purpose of $\mu_0$ is to produce LAC reconstructions
in correct units since the random initialization 
used for the neural network layers
serve to produce normalized outputs that are unit less. 

During back-propagation, each process computes the 
gradient of $L\left(\Omega_k; \gamma\right)$ 
with respect to the vector of network parameters, $\gamma$.
This gradient is another vector that is denoted by 
$\nabla_{\gamma}L\left(\Omega_k; \gamma\right)$
whose $l^{th}$ element is the partial derivative 
$\partial L\left(\Omega_k; \gamma\right)/\partial \gamma_l$
that is given by,
\begin{equation}
    \label{eq:partiald}
    \frac{\partial L\left(\Omega_k; \gamma\right)}{\partial \gamma_l}
    = \frac{1}{\vert\Omega_k\vert}\sum_{i\in\Omega_k}
    2 d_i (\gamma)
    \left(\sum_j w(r_{i,j})\frac{\partial \mathcal{M}(r_{i,j}; \gamma)}{\partial \gamma_l}\right),
\end{equation}
where $d_i(\gamma)$ is defined in equation \eqref{eq:mainsqdist}.
Note that equation \eqref{eq:partiald} is not
explicitly implemented in code, but is instead automatically
computed using algorithmic differentiation in PyTorch. 




\subsection{Network Architecture}
The DINR network, $\mathcal{M}(r_{i,j}; \gamma)$, 
is the concatenation of the following blocks of layers,
\begin{enumerate}
    \item Normalize $r_{i,j}=\left(t_i, z_{i,j}, y_{i,j}, x_{i,j}\right)$ such that each normalized coordinate in $r_{i,j}$ 
    is between $-1$ and $1$. 
    Since our object is assumed to lie inside the cylindrical field-of-view
    shown in Fig. \ref{fig:mainfig}, we normalize using the minimum
    and maximum coordinate values of the cylindrical boundary.
    Let $\bar{r}_{i,j}$ denote the normalized coordinates.
    \item Gaussian random Fourier feature (GRFF) encoding layer
    \cite{Fourier_INR_NEURIPS2020}
    to map the coordinates $\bar{r}_{i,j}$ to GRFF features as,
    \begin{equation}
        \text{GRFF}(\bar{r}_{i,j}) = 
        \begin{bmatrix}
            \cos\left(2\pi B \bar{r}^T_{i,j}\right) \\
            \sin\left(2\pi B \bar{r}^T_{i,j}\right)
        \end{bmatrix}^T
    \end{equation}
    where $T$ denotes transpose,  $\bar{r}^{T}_{i,j}$ is a column vector, 
    $B$ is a $C \times 4$ matrix of random numbers.
    Each element along the $1^{st}$ column of $B$ is 
    sampled from a Gaussian distribution with zero mean 
    and standard deviation of $\sigma_t$.
    Elements along the $2^{nd}$, $3^{rd}$, and $4^{th}$ columns of $B$
    are sampled from a Gaussian distribution with zero mean
    and standard deviation of $\sigma_s$.
    The elements of $B$ are not modified during training of 
    $\mathcal{M}(r_{i,j}; \gamma)$.
    An increasing value for $\sigma_s$ leads to
    increasing sharpness and noise of the DINR reconstruction 
    along the three spatial dimensions and vice versa.
    Similarly, increasing $\sigma_t$ leads to increasing 
    sharpness and noise of the DINR reconstruction along the time dimension
    and vice versa. 
    Thus, the value of $\sigma_s$ and $\sigma_t$ are important parameters
    that trade off sharpness with noise and spurious artifacts.
    \item The GRFF outputs of length $2C$ are then input to a sequence
    of $L$ fully connected (FC) linear layers.
    Each FC layer is followed by a 
    Swish activation function \cite{swish_ramachandran2017}.
    The number of input and output channels
    for each FC layer is $2C$.
    \item At the end, we have a FC layer to map the $2C$ number of input 
    channels to a single scalar value that is the object reconstruction
    at coordinate $r_{i,j}$. We multiply this value by $\mu_0$ 
    to convert it to LAC reconstruction units.
    We do not use an activation function for this last FC layer.
\end{enumerate}
Schematics of the network architecture and the training loop 
are provided in the supplementary figure Fig. \ref{fig:nnarch_train}.

\subsection{Training Parameters}
For the experimental data reconstruction in Fig. \ref{fig:deben202303}, 
we set $\sigma_s=0.5$ and $\sigma_t=0.1$.
For the experimental data reconstruction in Fig. \ref{fig:deben202310}, 
we set $\sigma_s=5.0$ and $\sigma_t=0.1$.
If $\sigma_t$ is progressively increased beyond a certain threshold,
we notice artifacts where the spatial features of the object 
seem to also rotate between subsequent time steps.
To get a stable reconstruction of the object,
we determined that $\sigma_t$ needs to be sufficiently small.
For our experimental data reconstructions, a single value 
of $\sigma_t=0.1$ was sufficient to get a stable reconstruction.
We recommend tuning of both $\sigma_s$ and $\sigma_t$ 
 by factors of $10$ starting from initial values of $1$.
Our goal was only to determine workable parameter values
that produced a minimum desired visual reconstruction quality. 
It is difficult to estimate the optimal values for $\sigma_s$ and $\sigma_t$
since they are application dependent.

The number of channels for the FC layers is set as $2C=256$.
The number of layers with the non-linear Swish activation
function is $L=5$.
The batch size per compute process is $\vert\Omega_k\vert=48$ 
in equation \eqref{eq:localoptfunc}.
We used $128$ number of compute processes to train the DINR
used for Fig. \ref{fig:deben202303} and \ref{fig:deben202310}.
The $128$ processes are distributed across $32$ HPC nodes each with $4$
Nvidia Tesla V100 GPUs such that each process runs on one GPU.
The learning rate is $0.001$ at the beginning of the training loop.
We use learning rate decay to progressively reduce the learning
rate by a multiplicative factor of $0.95$ after each epoch.



==> figs/deben202310/sec_recon.tex <==

% We use a Implicit Neural Representation (INR) network, 
% $\mathcal{M}_{\gamma}$, to 
% learn to predict the LAC, $\mu(x,y,z,t)$, from 
% an encoding of the time-space coordinates $(x,y,z,t)$.
% Here, $\gamma$ denotes the parameters (weights and bias terms)
% of the INR network $\mathcal{M}_{\gamma}$.
% We train the INR to predict $\mu(x,y,z,t)$ such that
% it satisfies equation \eqref{eq:logbeerslaw}.
% Thus, our objective is to solve the following optimization
% problem,
% \begin{equation}
% \label{eq:lossmin}
% \hat{\mu}\left(\cdot\right) = \arg\min_{\mu(\cdot)} 
% \sum_{i,j,k} w_{i,j,k}\left(y_{i,j,k}-\hat{f}_{i,j,k}\left(\mu(\cdot)\right)\right)^2,
% \end{equation}
% where the sum is over all measurements
% and $\mu(\cdot)$ is a function of the 
% coordinates $[x,y,z,t]^T$.

% The conventional approach to solving equation 
% \eqref{eq:lossmin} is to discretize $\mu(x,y,z,t)$
% over space and time.
% Each discretized element, indexed by $l$, 
% at a particular time instant $t_l$ 
% and space location $(x_l, y_l, z_l)$
% is called a voxel with a value of approximately
% $\mu\left(x_l,y_l,z_l,t_l\right)$.
% In volumetric space, we can sample $(x,y,z)$ such that the
% number of discrete elements along each of the three 
% dimensional axes is equal to the number of pixels 
% along any of the detector axes. 
% Similarly, we can sample $t$ such that the number
% of discrete samples equals the number of projection views.
% However, this approach is infeasible since 
% storage of just the LAC values, 
% $\mu\left(x_l,y_l,z_l,t_l\right)\,\forall\, l$,
% may exceed $10$ terabytes\footnote{For reference, 
% the maximum volatile memory in a state-of-the-art
% NVIDIA A100 GPU is $80GB$.
% The random access memory (RAM) in a typical modern 
% high-performance computing (HPC) system is also
% less than $1$ terabytes.
% } 
% Thus, reconstruction of a discrete voxel representation
% of $\mu\left(\cdot\right)$ is infeasible
% on modern compute systems. 
% Hence, we use a memory-efficient continuous time-space
% representation for $\mu(t,r)$ without the need 
% for discretization into voxels. 

% \begin{figure}[!thb]
% \begin{center}
% \includegraphics[width=4in]{figs/schematic.png}
% \end{center}
% \caption{\label{fig:sysdiag}
% }
% \end{figure}

% \begin{algorithm}
% \caption{One iteration of training for $\mathcal{M}_{\gamma}\left(\cdot\right)$.}
% \label{alg:traininr}
% \begin{algorithmic}[1]
% \Require Initialized $\mathcal{M}_{\gamma}\left(\cdot\right)$, and number of processes, $N$.
% \Ensure Copy $\mathcal{M}_{\gamma}\left(\cdot\right)$
% to each process $n$.
% \For {$n$ in $1$ to $N$}
%     \For {$(i,j,k) \in \Omega_n$}
%         \State Create the set $\Psi_{i,j,k}$.
%         \State Compute $\hat{f}_{i,j,k}
%          \left(\mathcal{M}_{\gamma}(\cdot)\right)$ using 
%          equation \eqref{eq:logbeerslaw}.
%         \State $\mathcal{L}_n \Leftarrow
%             \sum_{(i,j,k)\in\Omega_n} \left(y_{k,i,j}-
%             \hat{f}_{i,j,k}
%             \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2$.
%             \State Back-propagate $\mathcal{L}_n$ to compute $\frac{\partial \mathcal{L}_n}{\partial \gamma_k}$.
%     \EndFor
% \EndFor
% \State Average the gradients as $\frac{\partial \mathcal{L}}{\partial \gamma_k} = 
% \frac{1}{N}\sum_{n=1}^N \frac{\partial \mathcal{L}_n}{\partial \gamma_k}$.  
% \State Broadcast the averaged gradient 
% $\frac{\partial \mathcal{L}}{\partial \gamma_k}$ to each process $n$.

% \For{$n$ in $1$ to $N$}
%     \State Update $\gamma \Leftarrow \mathrm{Adam}\left(\gamma, \frac{\partial \mathcal{L}}{\partial \gamma_k} \,\forall\, k\right)$. \Comment{ $\mathrm{Adam}$ is the optimizer.}
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% We use an implicit neural representation (INR) network
% to learn the time-space dependence of the 
% object's linear attenuation coefficient (LAC).
% Our INR takes the time coordinate, $t$, 
% and spatial location, $(x,y,z)$, as inputs 
% and learns to predict the LAC, $\mu(x,y,z,t)$.
% The first stage of the INR normalizes the coordinates 
% $(x,y,z,t)$ such that the coordinate value for each axis
% is in the range of $\left(-1, 1\right)$.
% The second stage encodes the normalized coordinates 
% using a Gaussian Fourier feature representation. 
% Lastly, a fully-connected neural network (FCNN)
% predicts the LAC, $\mu(x,y,z,t)$, 
% from the Fourier features of the normalized $(x,y,z,t)$.
% Mathematically, we represent our INR 
% as $\mu(x,y,z,t) = \mathcal{M}_\gamma \left(x,y,z,t\right)$,
% where $\nu$ is the parameter set (weights and biases) for the
% neural network $\mathcal{M}_\gamma\left(\cdot\right)$.
% We optimize the parameters $\gamma$ of the INR such that
% the following loss function is minimized,
% \begin{equation}
% \label{eq:nnmin}
% \hat{\gamma} = \arg\min_{\gamma} \sum_{i,j,k}
% w_{i,j,k}\left(y_{i,j,k}-\hat{f}_{i,j,k}
% \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2.
% \end{equation}

% We use several distributed parallel processes 
% to speed up neural network training.
% Each compute process has one dedicated GPU that is used
% to compute the loss and gradient via back-propagation.
% Also, each process maintains an identical copy of the neural
% network model and optimizer stages.
% A pseudo-code for the training loop is 
% shown in algorithm \ref{alg:traininr}. 
% In order to split the compute across several distributed GPUs,
% we randomly sample measurements to compute a local loss
% function at each process. 
% For a given iteration, 
% let $\Omega_n$ denote the set of all indices used to 
% compute the loss at process $n$. 
% Then, the local loss at the $n^{th}$ process is,
% \begin{equation}
% \label{eq:nodeloss}
% \mathcal{L}_n = 
% \sum_{(i,j,k)\in\Omega_n} \left(y_{k,i,j}-
% \hat{f}_{i,j,k}
% \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2.
% \end{equation}
% The set $\Omega_n$ is randomly chosen at each iteration
% to compute the gradient at each node. 
% The losses and gradients are averaged across all the processes
% and the averaged values are broadcasted back to each process.
% The averaged gradient is used to update the parameters 
% $\gamma$ within each process.
% We use the Adam optimization algorithm to update the 
% parameters of the INR at each iteration.





==> figs/deben202310/sec_result.tex <==
\section{Results}

We evaluate DINR on both experimental and simulated datasets. 
For the experimental data, we used an X-ray CT scanner 
called Zeiss Xradia 510 Versa to perform 
in-situ 4DCT experiments of two samples under compression. 
A Deben CT5000 in-situ loadcell testing stage 
(Deben UK Ltd., United Kingdom) was used to 
perform in-situ compression during 
4DCT data acquisition on the Versa.
We performed in-situ 4DCT of crack propagation
in a SiC cylindrical sample and feature deformation
in a polydimethylsiloxane ``log pile'' sample \cite{osti_1871381}.
For ablation studies and 
a more rigorous quantitative evaluation, 
we used LLNL D4DCT dataset \cite{MPMDataset}, a simulated dataset 
for reconstruction of object deformation under mechanical loads over time. 
For simulation of CT projections, we used Livermore Tomography Tools (LTT) \cite{LTT} 
and Livermore AI Projector (LEAP) \cite{LEAPCT}. 
We provide image quality metrics 
for quantitative evaluation of the reconstruction as well as
comparison with state-of-the-art methods. 

\subsection{Experimental Data Evaluation}
%The stage is contained within a cylindrical carbon fiber envelope, which must be considered when performing flat field correction as the envelope contributes to X-ray attenuation.
We used an additive manufacturing technique called 
direct ink writing (DIW) to fabricate a polydimethylsiloxane 
``log-pile'' sample that is shown in Fig. \ref{fig:debendata} (a).
The log pile sample is comprised of several layers of strands;
between adjacent layers, the strands are rotated by $90^{\circ}$.
The distance between adjacent layers is approximately $0.750$ mm.
%Separating the siloxane from the steel anvils of the Deben stage 
%are disks of soft plastic that are approximately $1$ mm in thickness.
The second SiC sample shown in Fig. \ref{fig:debendata} (b) 
consists of two vertically stacked Silicon Carbide (SiC)
cylinders (or ``pucks'') made by binder jetting
that is also an additive manufacturing technique. 
The stacked pucks were approximately $8$ mm in diameter 
and approximately $2.8$ mm in height.
%Separating the pucks from the steel anvils on either side 
%of the Deben stage are $2$-mm thick plastic disks. 

\newcommand{\debmarhsp}{\hspace{-0.15in}}
\makeatletter
\define@key{Gin}{debmarfig}[true]{%
    \edef\@tempa{{Gin}{width=0.7in}}%
    \expandafter\setkeys\@tempa
}
\makeatother
\makeatletter
\define@key{Gin}{debmariso}[true]{%
    % https://tex.stackexchange.com/questions/57418/crop-an-inserted-image
    % Answer: [trim={left bottom right top},clip]
    %\edef\@tempa{{Gin}{trim={150px 350px 150px 350px},clip,width=0.8in,height=0.7in}}%
    \edef\@tempa{{Gin}{width=0.8in,height=0.8in}}%
    \expandafter\setkeys\@tempa
}
\makeatother

\begin{figure*}[!htb]
\begin{center}
\begin{tabular}{cccc}
\includegraphics[height=0.7in]{figs/debendata/Silicone-Truss.jpg} &
\includegraphics[height=0.7in]{figs/debendata/SiC-crop.png} &
\includegraphics[height=0.7in]{figs/debendata/Deben.jpg} &
\includegraphics[height=0.7in]{figs/debendata/Deben-Versa.jpg} \\
(a) Log-pile & (b) SiC & (c) Deben stage & (d) Zeiss Xradia 510 Versa \vspace{0.05in}\\
\end{tabular}
\includegraphics[width=4.7in]{figs/debendata/deb03_proj_cr0.png}\\
\includegraphics[width=4.7in]{figs/debendata/deb03_proj_cr1.png}\\
\vspace{-0.1in}
(e) X-ray projection images for the log pile sample.\vspace{0.05in}\\
\includegraphics[width=4.7in]{figs/debendata/deb10_proj_cr0.png}\\
\includegraphics[width=4.7in]{figs/debendata/deb10_proj_cr1.png}\\
\vspace{-0.1in}
(f) X-ray projection images for the SiC sample.\\
\end{center}
\caption{\label{fig:debendata}
4DCT of samples under compression in a Deben stage
that is mounted in a cone-beam X-ray CT system.
(a) and (b) show the log-pile and SiC samples 
used for the 4DCT scans. 
(c) is the Deben stage used for in-situ compression
of (a) and (b).
(d) is the Zeiss Xradia 510 Versa X-ray scanner 
that is used for cone-beam 4DCT.
(e) and (f) show the X-ray projection images 
of (a) and (b) respectively at different view angles. 
$T_m$ in the column labels of (e, f)
indicates the time of the projection images 
at the $m^{th}$ view.
In (e, f), the $2^{nd}$ row zooms into the images
in the $1^{st}$ row.
The green rectangle in the $t=0$ image at the top-side
of either (e) or (f) shows the location of this zoomed area.
}
\end{figure*}

\begin{figure*}[!htb]
\begin{center}
\hspace{-0.2in}
\includegraphics[width=4.6in]{figs/deben202303/deb03_TimeFrames_0.png} \\
\hspace{-0.2in}
\includegraphics[width=4.6in]{figs/deben202303/deb03_TimeFrames_1.png} \\
\hspace{-0.1in}
\includegraphics[width=4.6in]{figs/deben202303/deb03_TimeFrames_2.png} \\
(a) Sequence of time frames reconstructed using DINR.
\hspace{-0.1in}
\includegraphics[width=4.6in]{figs/deben202303/deb03_dynvsstat.png} \\
(b) Comparison between 
FDK (conventional 4DCT) and DINR (ours). \\
\end{center}
\caption{\label{fig:deben202303}
4DCT reconstruction of the log-pile sample
(Fig. \ref{fig:debendata} (a)).
(a) shows the 3D ISO surface of the 4D reconstruction
and the cross-section images of the LAC 
using the high-resolution DINR at various time indices. 
(b) is a reconstruction comparison of the 
cross-section images of the LAC between the 
conventional 4D FDK and our DINR approach.
The PSNR/SSIM values are embedded 
in the images of (b).
The high-resolution DINR images are the best
visual match for the ground-truth while also
producing the highest PSNR and SSIM.
}
\end{figure*}

%\makeatother
%\makeatletter
%\define@key{Gin}{deboctiso}[true]{%
%    % https://tex.stackexchange.com/questions/57418/crop-an-inserted-image
%    % Answer: [trim={left bottom right top},clip]
%    \edef\@tempa{{Gin}{trim={200px 200px 200px 200px},clip,width=0.8in,height=0.7in}}%
%    \expandafter\setkeys\@tempa
%}
%\makeatother
\begin{figure}[!thb]
\begin{center}
\includegraphics[width=4.5in]{figs/deben202310/deb10_3DAMIP_0.png}\\
\includegraphics[width=4.5in]{figs/deben202310/deb10_3DAMIP_1.png}\\
(a) 3D renderings of the high-resolution DINR reconstruction. \\
\hspace{-0.1in}
\includegraphics[width=4.5in]{figs/deben202310/deb10_dyninr_0.png}\\
\hspace{-0.15in}
\includegraphics[width=4.5in]{figs/deben202310/deb10_dyninr_1.png}\\
\hspace{-0.15in}
\includegraphics[width=4.5in]{figs/deben202310/deb10_dyninr_2.png}\\
(b) 4DCT reconstructions of the LAC using DINR.
\vspace{0.02in} \\
\includegraphics[width=4.5in]{figs/deben202310/deb10_dynfbp_3.png}\\
(c) Conventional 2-frame and 4-frame FDK reconstruction.
\vspace{0.1in} \\
\end{center}
\caption{\label{fig:deben202310}
4DCT reconstruction of the SiC sample (Fig. \ref{fig:debendata} (b)).
(a) shows the 3D AMIP volumes of the high resolution 
4D DINR reconstruction with clearly resolved 
propagation of cracks over time. 
(b) shows the high and low resolution DINR reconstruction
of a cross-axial volume slice at different time indices.
The low resolution DINR is unable to clearly resolve the cracks.
The high resolution DINR produces the best reconstruction that
clearly resolves the cracks at all times.
The first two images and the last four images in
(c) show the 2-frame FDK and the 4-frame FDK 
reconstructions respectively.
The 2-frame FDK suffers from motion blur while 
the 4-frame FDK has substantial limited angle artifacts.
}
\end{figure}


\begin{figure}[!htb]
\centering
\begin{subfigure}[b]{0.99\textwidth}
   \includegraphics[width=1\linewidth]{figs/figure_MPM_512_128_results_01.pdf}
   \caption{Reconstruction of first and last time frames for S08\_005}
   \label{fig:mpm1} 
\end{subfigure}

\begin{subfigure}[b]{0.99\textwidth}
   \includegraphics[width=1\linewidth]{figs/figure_MPM_512_128_results_02.pdf}
   \caption{Reconstruction of first and last time frames for S04\_018}
   \label{fig:mpm2} 
\end{subfigure}

\begin{subfigure}{.55\textwidth}
  \centering
   \includegraphics[width=1\linewidth]{figs/figure_MPM_512_128_psnr.pdf}
   \caption{Average PSNRs}
   \label{fig:mpm_psnr}
\end{subfigure}%
\hfill
\begin{subfigure}{.43\textwidth}
  \centering
   \includegraphics[width=1\linewidth]{figs/figure_MPM_strong_scaling2.pdf}
   \caption{Strong Scaling}
   \label{fig:mpm_scaling}
\end{subfigure}
\caption{Qualitative and quantitative comparison 
of 4DCT reconstructions using simulated MPM datasets. 
(a, b) are visual comparisons between 
DINR and other state-of-the-art methods. 
(a) and (b) show the 4D reconstructions 
for the S08\_005 and S04\_018 MPM datasets. 
The $1^{st}$ row of (a, b) show the first time frame.
The $2^{nd}$ row of (a, b) show the last time frame. 
We used isosurface 3D visualization for DINR and PINR.  
For TIMBIR and 2-Frame FBP,  we instead used MIP 
volume rendering due to illegible isosurfaces.
(c) shows the average PSNRs between the reconstructions and ground-truth. 
The error bars in (c) indicate the minimum and maximum PSNRs. 
(d) demonstrates strong scaling of DINR as a function of the number 
of compute nodes and GPUs.}
\label{fig:mpm}
\end{figure}

For in-situ 4DCT, each sample in Fig. \ref{fig:debendata} (a, b)
is individually mounted in the Deben CT5000 in-situ 
loadcell testing stage shown in Fig. \ref{fig:debendata} (c).
We used plastic disk spacers to separate the samples
from the steel anvils of the Deben stage.
The Deben stage with the sample is then 
mounted in the Zeiss Xradia 510 Versa
X-ray scanner shown in Fig. \ref{fig:debendata} (d).
For the in-situ 4DCT compression experiments, 
each sample was compressed at a speed of $0.030$ mm/min.
The exposure time for each X-ray projection image was $10$ seconds.
Thus, the acquisition time for the $m^{th}$
projection in units of seconds is,
\begin{equation}
\label{eq:projtime}
T_m \approx 10m.    
\end{equation}
Note that each projection image corresponds to a different 
morphological structure during 
the dynamical evolution of the sample.
Since the object is also continuously rotating,
each projection image corresponds to a different view angle
of the object.
The shape of each projection image was $1024\times 1024$.
Hence, each projection image consists of $1048576$ pixels.
The pixel size for the projection images is $69.16$ microns.

In Fig. \ref{fig:debendata} (e), 
we show projection images at different view angles
of the log-pile sample such that the second row images 
zoom into a portion of the first row images.
The times and the corresponding indices for the projection images of 
Fig. \ref{fig:debendata} (e) are indicated by $T_m$
in the column labels.
We acquired $722$ X-ray projection images 
over two full rotations of $361^{\circ}$
and show the projection images at the time/view indices 
of $m = 0, 144, 288, 433, 577$ and $721$.
We observe buckling of the log-pile sample over time from different views
as the anvil of the Deben stage progressively 
compresses the sample from the bottom-side.
%During each acquisition of $361$ projections 
%spanning $360$ degrees of rotation, 
%the sample was compressed by approximately $2$ mm. 
The sample was compressed by approximately $4$ mm 
over the duration of the experiment.
The source to object (SOD) and source to detector distances (SDD)
were $80 mm$ and $140 mm$ respectively on the Versa.

The X-ray projection images of the SiC sample at different view angles
are shown in Fig. \ref{fig:debendata} (f) 
and the second row shows images that zoom into the first row images.
We acquired $200$ projection images over an angular rotation range of 
approximately $397.8$ degrees.
The total compression of the sample was approximately $1$ mm
over the duration of the $200$ views.
Fig. \ref{fig:debendata} (f) shows the projection images
at the time/view indices of $m = 0, 40, 80, 119, 159,$ and $199$.
We observe progressive crack propagation over time 
near the edges of the SiC sample in the projection images.
The source to object (SOD) and source to detector distances (SDD)
were $65mm$ and $325mm$ respectively for this scan.
The pixel size for the projection images is $34.58$ microns.

The conventional approach to 4DCT is to split the 
projection images into groups such that
each group of projections is reconstructed into one volumetric frame.
The projections in each group are from consecutive 
views or time indices without any overlap of indices between groups.
This approach to 4DCT relies on an assumption
of static object for the time duration of the projections within each group.
However, since each group may span hundreds to thousands of projection images,
we are only able to reconstruct samples with very slow dynamics
using this approach.
This limitation of conventional 4DCT is a characteristic 
of most existing analytical and iterative reconstruction 
algorithms \cite{kak1998, mohan2015timbir}.
Feldkamp-Davis-Kress (FDK) \cite{Feldkamp84_FDKrecon}
is one such analytical cone-beam reconstruction algorithm that is
used for experimental data comparisons.
Henceforth, we use the notation $K-$FDK to refer to 
$K$ number of FDK reconstructed time frames 
(each time frame is a volumetric reconstruction) 
from $K$ groups of projections respectively.

If the static assumption for the object 
is violated within any group of projections, 
we observe substantial motion artifacts and blur
in the reconstructed volumes.  
If the number of views in each group is reduced
to mitigate motion blur,
we instead observe substantial limited angle artifacts (streaks)
when the angular span of rotation reduces to less than $180^{\circ}$
for parallel-beam geometry.
For cone-beam, this limit is a variable that depends on the cone-angle,
but is generally a higher number that varies 
between $180^{\circ}$ and $360^{\circ}$.
The iterative TIMBIR algorithm \cite{mohan2015timbir} 
also suffers from the same limitation while also 
currently only supporting the parallel-beam CT geometry.
In contrast, DINR assumes a dynamic object that allows temporal 
changes for the object between subsequent projection images.
This property of DINR enables the reconstruction 
of objects with very fast dynamics.
Note that all our experimental data reconstructions 
are for the challenging cone-beam X-ray system geometry.


In Fig. \ref{fig:deben202303}, we demonstrate that only our high-resolution
DINR reconstruction is able to best resolve the strands of the log-pile
sample at various time indices. 
Here, high-resolution refers to reconstruction of volumes
using projection images without down-sampling 
at pixel sizes of $69.16\mu m$. 
The high-resolution DINR reconstruction at various time indices
is shown in Fig. \ref{fig:deben202303} (a).
We show reconstructions at the same time indices as the
projection images in Fig. \ref{fig:debendata} (e).
The various columns are at time
indices of $m = 0, 144, 288, 433, 577$ and $721$.
The $1^{st}$ row of Fig. \ref{fig:deben202303} (a) 
shows the 3D renderings of the isosurfaces 
(labeled as ISO in Fig. \ref{fig:deben202303} (a))
computed from the reconstructed volumes.
We used Napari \cite{napari_ahlers_2023} for generating isosurfaces.
Each ISO surface was produced from a volumetric reconstruction
of size $400 \times 1024 \times 1024$.
The $2^{nd}$ row of Fig. \ref{fig:deben202303} (a) zooms
into a portion of the isosurface renderings in the $1^{st}$ row.
The $3^{rd}$ row of Fig. \ref{fig:deben202303} (a) 
shows cross-axial slices of the reconstructed volumetric time frames.
These cross-axial images are in units of the 
linear attenuation coefficient (LAC)
given by the DINR output $\mathcal{M}(r_{i,j}$ multiplied by $\mu_0$
(from equation \eqref{eq:weightfactors}).
They are scaled between a minimum of $0 mm^{-1}$
and a maximum of $0.1 mm^{-1}$.
The DINR outputs are obtained by neural network inference
after training. 

To facilitate quantitative comparisons, 
we acquired static CT scans of the log-pile sample
prior to and after compression.
FDK reconstructions of the sample from 
these static CT scans are treated as the ground-truth
and shown along the $1^{st}$ column of Fig. \ref{fig:deben202303} (b).
We use these ground-truth images to compute the 
peak signal to noise ratio (PSNR) and structural similarity index (SSIM) 
metrics for quantitatively assessing the 
performance of various reconstruction approaches.
The PSNR (units of dB) and SSIM metrics are computed 
after min/max normalization
of the reconstructed images using the minimum and maximum values of the 
ground-truth images.

The conventional 2-FDK in the $2^{nd}$ 
column of Fig. \ref{fig:deben202303} (b)
uses FDK reconstructions of the first $361$ projection images 
as the first frame and that of the last $361$ projection images
as the last frame respectively.
Similarly, the 4-FDK in the $3^{rd}$ column shows FDK reconstructions 
of the first and the last $180$ number of projection images
as the first and last frames respectively.
The $2$-FDK, $4$-FDK, and $6$-FDK lead to very low fidelity
reconstructions with misplaced positioning of image features.
The dynamics or motion in the sample during the time span of each
frame for $2$-FDK causes significant motion blur.
With $4$-FDK and $6$-FDK, in addition to blur, we observe 
limited angle artifacts since the angular rotation 
is approximately $180^{\circ}$ and $120^{\circ}$ respectively.

We evaluate DINR for 4D reconstruction of the log-pile sample
under compression for two cases of low and high resolution 4DCT.
The low-resolution DINR reconstructions 
in the $5^{th}$ column of Fig. \ref{fig:deben202303} (b) 
are from projection images down-sampled by a factor of $8$.
Alternatively, the high-resolution DINR reconstructions
in the last column of Fig. \ref{fig:deben202303} (b) 
are from projection images without any down-sampling.
The advantage of the low-resolution DINR is the significantly lower
memory and compute costs due to the substantially smaller data size. 
However, this approach leads to severely blurred image features 
due to a $8\times$ reduction in pixel size.
Prior neural representation approaches including \cite{Reed2021} 
require substantial down-sampling of projection data
to meet the constraints of compute and memory. 
Unfortunately, such down-sampling may not be suitable for cases
where high-resolution is a fundamental necessity.
Among all approaches, the high-resolution DINR along the last column
produces the best reconstruction with the highest fidelity
and is the only method to accurately reconstruct
the strands of the log-pile sample.
The highest PSNR and SSIM is achieved by the high-resolution DINR
along each row of Fig. \ref{fig:deben202303} (b).
The pixel sizes of the projection images for the low
and high-resolution cases were $553.2\mu m$ and $69.16\mu m$ respectively


We demonstrate the effective reconstruction of crack propagation 
inside a SiC sample using DINR in Fig. \ref{fig:deben202310}.
Fig. \ref{fig:deben202310} (a) show 
3D renderings using attenuated maximum intensity projection (AMIP)
of the volumetric reconstructions at different time steps.
We use Napari \cite{napari_ahlers_2023} to generate the AMIP 3D renderings.
We show time frames from the 4DCT reconstruction at 
projection indices of $m = 0, 40, 80, 119, 159, $ and $199$. 
The times for these reconstructions directly correspond
to the morphology of the sample during the acquisition times 
of the projection images shown in Fig. \ref{fig:debendata} (f).

We show the high and low resolution
DINR reconstructions of a cross-axial slice 
for the SiC sample in Fig. \ref{fig:deben202310} (b).
These reconstructions are in units of LAC
similar to Fig. \ref{fig:deben202303} (b). 
The low resolution DINR reconstruction along the $3^{rd}$ row of  
Fig. \ref{fig:deben202310} (b) are reconstructions of 
projection images that are down-sampled by a 
factor of $8$ along each image dimension.
Due to the lower resolution, the low resolution DINR is unable
to clearly resolve the cracks, especially at later time steps.
The high-resolution DINR reconstructions in the $1^{st}$ and $2^{nd}$
rows of Fig. \ref{fig:deben202310} (b) produce substantially
improved reconstructions that clearly resolve 
the cracks at each time index.
In Fig. \ref{fig:deben202310} (c), we show the conventional 
$2$-FDK and $4$-FDK 4DCT reconstruction 
of a cross-axial volume slice.
The $2$-FDK shows reconstructed time frames from $2$ projection groups
each consisting of $100$ consecutive projection images.
The $4$-FDK shows reconstructed time frames from $4$ projection groups
each consisting of $50$ consecutive projection images.
None of the 4DCT reconstructions using FDK are able to clearly
resolve crack propagation due to insufficient temporal resolution.
$2$-FDK suffers from motion blur due to substantial crack 
propagation over $100$ views.
$4$-FDK produces limited angle artifacts
due to a rotation of approximately $99^{\circ}$
for the projections in each group.

\subsection{Simulated Data Evaluation}

For a quantitative performance analysis of DINR 
and other state-of-the-art methods for 4DCT reconstruction, 
we used a simulated dataset called LLNL D4DCT Datasets~\cite{MPMDataset}. 
This dataset was generated using the material point method (MPM)~\cite{MPM_CPDI2} to precisely simulate the deformation 
of a specific type of aluminum object, a 6061 aluminum alloy, 
for a range of object shapes and compression scenarios. 
For each dataset, the simulated volumes of object deformation over time 
are then voxelized into $360$ time frames. 
These MPM datasets span a range of volume resolutions 
and each dataset includes a subset of the total time frames. 
Among $157$ datasets of varying object shapes and compression scenarios
in LLNL D4DCT Datasets~\cite{MPMDataset}, 
we selected $6$ datasets for our experiments: 
S03\_001, S03\_008, S04\_009, S04\_018, S05\_700, and S08\_005. 

We compare state-of-the-art 4DCT reconstruction methods
against DINR at two volumetric resolutions with pixel sizes 
of $2$mm and $0.05$mm in Fig. \ref{fig:mpm}. 
For the lower resolution dataset ($2$mm pixel size), 
we simulated $91$ volumetric time frames of size $128^3$.
For the higher resolution dataset ($0.05$mm pixel size), 
we simulated $181$ volumetric time frames of size $512^3$.
Next, we simulated CT projection images from the time frames
such that the $m^{th}$ image was simulated from the $m^{th}$ time frame.
This ensures each projection image is generated from a 
unique volumetric time frame to simulate 4DCT of a 
continuously deforming object over time.
The rotation angular range for both the low and high resolution
scenarios was $180^{\circ}$. 
The projection geometry is parallel-beam for CT data simulation. 
We also simulate $0.1\%$ Poisson noise in the X-ray transmission space
(negative logarithm of projections).
We used the Livermore Tomography Tools (LTT) \cite{LTT} 
software library for simulation of 4DCT data. 
The reader is advised to consult the 
dataset website \cite{MPMDataset} for more details. 

We compare DINR against two state-of-the-art 4DCT reconstruction methods:
TIMBIR~\cite{mohan2015timbir} and Parametric INR (PINR)~\cite{Reed2021}. 
We also performed limited-angle CT (90\degree) reconstruction 
using 2-frame filtered back projection (FBP). 
Figure~\ref{fig:mpm} (a) and (b) shows 3D visualizations of 
the 4D reconstruction for S03\_001 and S04\_018 
using DINR, PINR, TIMBIR, and 2-Frame FBP. 
We used isosurface 3D visualization for DINR and PINR.
For TIMBIR and FBP, we were unable to study isosurfaces 
due to the presence of severe artifacts. 
Hence, we visualized TIMBIR and FBP 
using maximum intensity projection (MIP)-based volume rendering.
DINR-128 and PINR-128 were reconstructed from the lower resolution 
projection data with pixel size of $2$mm.
DINR-512 was reconstructed from the higher resolution
projection data with pixel size of $0.05$mm.
Compared to the ground-truth, 
DINR-512 produces the best visual quality of reconstruction
for both S03\_001 and S04\_018.
Reconstructions using TIMBIR are barely recognizable 
since it is optimized for sparse views with interleaved angular sampling. 
However, our scenario is more challenging due to limited-angle sampling. 
For TIMBIR, we carefully tuned the regularization parameters 
to obtain the best visual reconstruction quality. 
For more reconstructions that depict object deformation across time, 
please refer to the images in the supplementary section. 

To facilitate a quantitative comparison between the low
and high resolution reconstructions, we down-sampled the 
DINR-512 reconstructed volumes from $512^3$ to $128^3$.
This also serves to demonstrate the superior reconstruction 
of lower resolution features using DINR-512.
We report the PSNRs between each method's reconstruction 
and ground-truth in Fig. \ref{fig:mpm} (c). 
We show the PSNRs averaged over $10$ volumes 
that are equally spaced across time frames. 
DINR-512 produces the highest PSNR for all datasets.
While the performance benefits of DINR-128 compared to PINR-128
is inconclusive, we observed that
the DINR-128 reconstructions contain fewer artifacts 
on the surface of the object. 


We experimentally validated strong scaling of DINR 
using a GPU compute cluster \cite{LC_Lassen} 
with 4 NVIDIA V100 GPUs per compute node. 
We report speedup for $30$ epochs of neural network 
optimization across different number of GPUs and compute nodes.
We measured the total run times as the number of nodes 
was varied from 4 (16 GPUs) to 32 (128 GPUs). 
If $D$ is the number of nodes, then we define speedup
as the ratio of the runtime using one node and $D$ nodes. 
As shown in Figure~\ref{fig:mpm} (d), 
the scaling results demonstrate strong scalability 
of DINR due to effective distribution of the optimization 
across multiple nodes and GPUs. 

==> sec_recon.tex <==

% We use a Implicit Neural Representation (INR) network, 
% $\mathcal{M}_{\gamma}$, to 
% learn to predict the LAC, $\mu(x,y,z,t)$, from 
% an encoding of the time-space coordinates $(x,y,z,t)$.
% Here, $\gamma$ denotes the parameters (weights and bias terms)
% of the INR network $\mathcal{M}_{\gamma}$.
% We train the INR to predict $\mu(x,y,z,t)$ such that
% it satisfies equation \eqref{eq:logbeerslaw}.
% Thus, our objective is to solve the following optimization
% problem,
% \begin{equation}
% \label{eq:lossmin}
% \hat{\mu}\left(\cdot\right) = \arg\min_{\mu(\cdot)} 
% \sum_{i,j,k} w_{i,j,k}\left(y_{i,j,k}-\hat{f}_{i,j,k}\left(\mu(\cdot)\right)\right)^2,
% \end{equation}
% where the sum is over all measurements
% and $\mu(\cdot)$ is a function of the 
% coordinates $[x,y,z,t]^T$.

% The conventional approach to solving equation 
% \eqref{eq:lossmin} is to discretize $\mu(x,y,z,t)$
% over space and time.
% Each discretized element, indexed by $l$, 
% at a particular time instant $t_l$ 
% and space location $(x_l, y_l, z_l)$
% is called a voxel with a value of approximately
% $\mu\left(x_l,y_l,z_l,t_l\right)$.
% In volumetric space, we can sample $(x,y,z)$ such that the
% number of discrete elements along each of the three 
% dimensional axes is equal to the number of pixels 
% along any of the detector axes. 
% Similarly, we can sample $t$ such that the number
% of discrete samples equals the number of projection views.
% However, this approach is infeasible since 
% storage of just the LAC values, 
% $\mu\left(x_l,y_l,z_l,t_l\right)\,\forall\, l$,
% may exceed $10$ terabytes\footnote{For reference, 
% the maximum volatile memory in a state-of-the-art
% NVIDIA A100 GPU is $80GB$.
% The random access memory (RAM) in a typical modern 
% high-performance computing (HPC) system is also
% less than $1$ terabytes.
% } 
% Thus, reconstruction of a discrete voxel representation
% of $\mu\left(\cdot\right)$ is infeasible
% on modern compute systems. 
% Hence, we use a memory-efficient continuous time-space
% representation for $\mu(t,r)$ without the need 
% for discretization into voxels. 

% \begin{figure}[!thb]
% \begin{center}
% \includegraphics[width=4in]{figs/schematic.png}
% \end{center}
% \caption{\label{fig:sysdiag}
% }
% \end{figure}

% \begin{algorithm}
% \caption{One iteration of training for $\mathcal{M}_{\gamma}\left(\cdot\right)$.}
% \label{alg:traininr}
% \begin{algorithmic}[1]
% \Require Initialized $\mathcal{M}_{\gamma}\left(\cdot\right)$, and number of processes, $N$.
% \Ensure Copy $\mathcal{M}_{\gamma}\left(\cdot\right)$
% to each process $n$.
% \For {$n$ in $1$ to $N$}
%     \For {$(i,j,k) \in \Omega_n$}
%         \State Create the set $\Psi_{i,j,k}$.
%         \State Compute $\hat{f}_{i,j,k}
%          \left(\mathcal{M}_{\gamma}(\cdot)\right)$ using 
%          equation \eqref{eq:logbeerslaw}.
%         \State $\mathcal{L}_n \Leftarrow
%             \sum_{(i,j,k)\in\Omega_n} \left(y_{k,i,j}-
%             \hat{f}_{i,j,k}
%             \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2$.
%             \State Back-propagate $\mathcal{L}_n$ to compute $\frac{\partial \mathcal{L}_n}{\partial \gamma_k}$.
%     \EndFor
% \EndFor
% \State Average the gradients as $\frac{\partial \mathcal{L}}{\partial \gamma_k} = 
% \frac{1}{N}\sum_{n=1}^N \frac{\partial \mathcal{L}_n}{\partial \gamma_k}$.  
% \State Broadcast the averaged gradient 
% $\frac{\partial \mathcal{L}}{\partial \gamma_k}$ to each process $n$.

% \For{$n$ in $1$ to $N$}
%     \State Update $\gamma \Leftarrow \mathrm{Adam}\left(\gamma, \frac{\partial \mathcal{L}}{\partial \gamma_k} \,\forall\, k\right)$. \Comment{ $\mathrm{Adam}$ is the optimizer.}
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% We use an implicit neural representation (INR) network
% to learn the time-space dependence of the 
% object's linear attenuation coefficient (LAC).
% Our INR takes the time coordinate, $t$, 
% and spatial location, $(x,y,z)$, as inputs 
% and learns to predict the LAC, $\mu(x,y,z,t)$.
% The first stage of the INR normalizes the coordinates 
% $(x,y,z,t)$ such that the coordinate value for each axis
% is in the range of $\left(-1, 1\right)$.
% The second stage encodes the normalized coordinates 
% using a Gaussian Fourier feature representation. 
% Lastly, a fully-connected neural network (FCNN)
% predicts the LAC, $\mu(x,y,z,t)$, 
% from the Fourier features of the normalized $(x,y,z,t)$.
% Mathematically, we represent our INR 
% as $\mu(x,y,z,t) = \mathcal{M}_\gamma \left(x,y,z,t\right)$,
% where $\nu$ is the parameter set (weights and biases) for the
% neural network $\mathcal{M}_\gamma\left(\cdot\right)$.
% We optimize the parameters $\gamma$ of the INR such that
% the following loss function is minimized,
% \begin{equation}
% \label{eq:nnmin}
% \hat{\gamma} = \arg\min_{\gamma} \sum_{i,j,k}
% w_{i,j,k}\left(y_{i,j,k}-\hat{f}_{i,j,k}
% \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2.
% \end{equation}

% We use several distributed parallel processes 
% to speed up neural network training.
% Each compute process has one dedicated GPU that is used
% to compute the loss and gradient via back-propagation.
% Also, each process maintains an identical copy of the neural
% network model and optimizer stages.
% A pseudo-code for the training loop is 
% shown in algorithm \ref{alg:traininr}. 
% In order to split the compute across several distributed GPUs,
% we randomly sample measurements to compute a local loss
% function at each process. 
% For a given iteration, 
% let $\Omega_n$ denote the set of all indices used to 
% compute the loss at process $n$. 
% Then, the local loss at the $n^{th}$ process is,
% \begin{equation}
% \label{eq:nodeloss}
% \mathcal{L}_n = 
% \sum_{(i,j,k)\in\Omega_n} \left(y_{k,i,j}-
% \hat{f}_{i,j,k}
% \left(\mathcal{M}_{\gamma}(\cdot)\right)\right)^2.
% \end{equation}
% The set $\Omega_n$ is randomly chosen at each iteration
% to compute the gradient at each node. 
% The losses and gradients are averaged across all the processes
% and the averaged values are broadcasted back to each process.
% The averaged gradient is used to update the parameters 
% $\gamma$ within each process.
% We use the Adam optimization algorithm to update the 
% parameters of the INR at each iteration.




